MindfulDiary: Harnessing Large Language Model to Support Psychiatric Patients' Journaling

In the mental health domain, Large Language Models (LLMs) offer promising new opportunities, though their inherent complexity and low controllability have raised questions about their suitability in clinical settings. We present MindfulDiary, a mobile journaling app incorporating an LLM to help psychiatric patients document daily experiences through conversation. Designed in collaboration with mental health professionals (MHPs), MindfulDiary takes a state-based approach to safely comply with the experts' guidelines while carrying on free-form conversations. Through a four-week field study involving 28 patients with major depressive disorder and five psychiatrists, we found that MindfulDiary supported patients in consistently enriching their daily records and helped psychiatrists better empathize with their patients through an understanding of their thoughts and daily contexts. Drawing on these findings, we discuss the implications of leveraging LLMs in the mental health domain, bridging the technical feasibility and their integration into clinical settings.

==> contents/backup.tex <==


%https://www.nami.org/About-Mental-Illness/Treatments/Types-of-Mental-Health-Professionals
%우리 프로그램 참여한 전문가: Mental Health Professionals
%상담사: Clinicians
%의사(전공의): Psychiatrists
%Mental Health Support
%Mental Health
%Clinical Mental Health Setting
%%도메인 관련 내용 추가하기!
%Patient Journaling의 문제 => LLM이 주는 새로운 기회 => LLM의 의학분야 적용에의 난점 => 우리가 한 것
\section{Introduction}
A journal is a form of writing that records an individual's past events, thoughts, and feelings. What makes a journal unique is that, the person who writes the journal is usually the only reader. This characteristic makes journals a place where writers can freely express worries, thoughts, and feelings without being judged by others~\cite{Travers2011, Ullrich2002}. In clinical mental health, journals possess significant potential as they contain the patient's daily experiences, symptoms, and other unattainable information during the hospital appointment. This data enriches the understanding of the patient's condition, ultimately enhancing the quality of treatment provided~\cite{figueiredo2020patient, zhu2016sharing}.

%이러한 journal은 




In recent years, the potential of language models in healthcare, especially within the mental health domain, has garnered significant attention. For instance, chatbots dedicated to mental health support can offer enhanced accessibility to interventions like cognitive behavioral therapy~\cite{woebot, 10.2196/12106, fulmer2018using}, behavioral reinforcement~\cite{10.2196/12106}, and expressive writing~\cite{park_chatbot}, making support available anytime and anywhere~\cite{park_chatbot, cameron2019assessing}. Moreover, language models not only benefit patients but also serve as valuable tools for clinicians and therapists. They assist in summarizing and analyzing psychotherapy session notes~\cite{perlich2015automatic}, streamline the challenging task of identifying emotions in counseling data, and help therapists deepen their understanding of patients, evaluate potential interventions, and monitor patient progress more effectively~\cite{sentiment_understand, goldberg2020machine, NLP11}.

Recent advancements in pre-trained large language models (LLMs) have expanded the capabilities of natural language comprehension and generation. Traditional mental health chatbots were usually retrieval-based, functioning within a fixed structure~\cite{ABDALRAZAQ2019103978}. Such systems inherently struggle with adaptability and potentially fail when encountering unforeseen contexts or messages missing from the database~\cite{chatbot_review21, 10.1109/icac347590.2019.9036844}. Conversely, chatbots driven by LLMs, offer dynamic responses across multiple domains and tasks~\cite{bae2022building, roller-etal-2021-recipes, brown2020language}. This approach mitigates the limitations of retrieval-based models, promising a nuanced understanding of users in mental health, encompassing a diverse range of topics and individual traits.

While the LLMs present possibilities, they also come with inherent limitations and concerns. A major concern is the unpredictability and inconsistency of the outputs these models produce, leading to potential risks of generating unintended or inaccurate responses~\cite{farhat2023chatgpt, chatbot_review21, npj21}. These limitations emphasize the necessity of approaching LLMs with caution, especially in mental health contexts that require a delicate balance of sensitivity, accuracy, and safety. Although it might not be wise to depend solely on LLMs for mental health, previous research suggests integrating them into established healthcare systems. Within these systems, they can support and complement existing clinical practices~\cite{npj21}.

Building on this notion of integration, it's crucial for designers and engineers to collaborate with domain experts. This collaboration allows for a deeper understanding of LLMs' capabilities and aligning expectations. Furthermore, such synergy can help mitigate over-reliance on technology and address the clinically relevant challenges~\cite{10.1145/3564752}.



In this work, we present MindfulDiary, a mobile conversational AI for journaling that enables patients to record their daily experiences and thoughts through conversation. MindfulDiary incorporates LLMs to generate a response, prompting them differently according to the conversational phase. The conversation records are automatically summarized and presented on a clinician's dashboard so psychiatrists or clinicians can obtain insights about the patient. A multi-disciplinary research team, which included HCI researchers, engineers, and mental health professionals (i.e., psychiatrists and clinicians), carried out this project. We iteratively designed MindfulDiary, drawing insights from focus group interviews, expert evaluations of the chatbot's behaviors, and pilot studies.

To examine how patients interact with MindfulDiary, we conducted a four-week field study with 28 psychiatric patients and five psychiatrists at a university hospital. Patients performed journaling with MindfulDiary for four weeks, and their primary psychiatrists used the clinician's dashboard when they met their patients. The study revealed that the versatility, narrative-building capability, and diverse perspectives provided by MindfulDiary assist patients in consistently enriching their daily records. Furthermore, MindfulDiary supported patients in overcoming the challenges of detailed record-keeping and expression, often hindered by feelings of apathy and cognitive burdens. Notably, the enriched records from MindfulDiary, previously unattainable, provided psychiatrists with deeper insights, enhancing their understanding and empathy towards patients. Based on the findings, we discuss both the potential of LLMs' conversational abilities to aid in patient record-keeping within clinical mental health settings and suggestions for their responsible integration into these environments.

\npstart{The contributions from our research are as follows:}
\begin{enumerate}[leftmargin=*, itemsep=4pt, topsep=0pt]
    \item We present MindfulDiary, an LLM-driven journal designed to document psychiatric patients' daily experiences through naturalistic conversation developed in collaboration with mental health professionals.
    \item From a 28-day field study involving 28 patients and five psychiatrists, we provide empirical findings on how MindfulDiary supports patients in maintaining daily logs and assists psychiatrists in monitoring and comprehending patient states.
    \item Drawing from the design process of MindfulDiary and the findings of our deployment study, we outline key considerations and share lessons learned for the design and implementation of LLM's conversational capability in clinical mental health settings.
\end{enumerate}

%참고: This work forms part of a three-year, multi-disciplinary research collaboration thatcomprises a diverse team of researchers and developers with backgrounds in ML, Clinical Psychology,HCI, Design, Engineering and Data Compliance. Jointly, we investigate identified AI challenges in thecontext of SilverCloud Health0F1, an established iCBT platform for the treatment of depression, anxiety, andfunctional impairments [86].

%The authors of this paper include an HCI researcher, an AI engineer, and a university hospital professor. Additionally, ten medical professionals, comprising counselors and psychiatrists, collaborated on the development and deployment of MindfulDiary over eight months. The university hospital where this research took place is recognized as a tertiary hospital in Korea. In our work, we aimed to uncover the potential advantages and challenges of using LLMs in a clinical setting for mental health care, illustrated through the development and implementation of MindfulDiary. The subsequent section presents the formative study that served as the basis for the initial concept and design of our language model-based program.

% As underscored in Human-AI interaction design guidelines, the emphasis shouldn't solely be on "what new capabilities technologies like LLMs can offer" but rather on their intended purpose and the best way to utilize them in the given context~\cite{googlepair}. 

% Through the design of MindfulDiary, we explored how LLM capabilities, such as natural language understanding, summarization, and generation, can play a role in the mental health clinical setting. We conducted a field deployment study over four weeks with 28 patients and five psychiatrists. Through this, we were able to understand how the LLM-integrated MindfulDiary can be utilized in recording patients' daily logging and assisting mental health professionals in understanding and diagnosing patients.





%https://www.nami.org/About-Mental-Illness/Treatments/Types-of-Mental-Health-Professionals
%우리 프로그램 참여한 전문가: Mental Health Professionals
%상담사: Clinicians
%의사(전공의): Psychiatrists
%Mental Health Support
%Mental Health
%Clinical Mental Health Setting

\section{Introduction}
%%도메인 관련 내용 추가하기!
%Patient Journaling의 문제 => LLM이 주는 새로운 기회 => LLM의 의학분야 적용에의 난점 => 우리가 한 것


In recent years, the potential of language models in healthcare, especially within the mental health domain, has garnered significant attention. For instance, chatbots dedicated to mental health support can offer enhanced accessibility to interventions like cognitive behavioral therapy~\cite{woebot, 10.2196/12106, fulmer2018using}, behavioral reinforcement~\cite{10.2196/12106}, and expressive writing~\cite{park_chatbot}, making support available anytime and anywhere~\cite{park_chatbot, cameron2019assessing}. Moreover, language models not only benefit patients but also serve as valuable tools for clinicians and therapists. They assist in summarizing and analyzing psychotherapy session notes~\cite{perlich2015automatic}, streamline the challenging task of identifying emotions in counseling data, and help therapists deepen their understanding of patients, evaluate potential interventions, and monitor patient progress more effectively~\cite{sentiment_understand, goldberg2020machine, NLP11}.

Recent advancements in pre-trained large language models (LLMs) have expanded the capabilities of natural language comprehension and generation. Traditional mental health chatbots were usually retrieval-based, functioning within a fixed structure~\cite{ABDALRAZAQ2019103978}. Such systems inherently struggle with adaptability and potentially fail when encountering unforeseen contexts or messages missing from the database~\cite{chatbot_review21, 10.1109/icac347590.2019.9036844}. Conversely, chatbots driven by LLMs, offer dynamic responses across multiple domains and tasks~\cite{bae2022building, roller-etal-2021-recipes, brown2020language}. This approach mitigates the limitations of retrieval-based models, promising a nuanced understanding of users in mental health, encompassing a diverse range of topics and individual traits.

While the LLMs present possibilities, they also come with inherent limitations and concerns. A major concern is the unpredictability and inconsistency of the outputs these models produce, leading to potential risks of generating unintended or inaccurate responses~\cite{farhat2023chatgpt, chatbot_review21, npj21}. These limitations emphasize the necessity of approaching LLMs with caution, especially in mental health contexts that require a delicate balance of sensitivity, accuracy, and safety. Although it might not be wise to depend solely on LLMs for mental health, previous research suggests integrating them into established healthcare systems. Within these systems, they can support and complement existing clinical practices~\cite{npj21}.
% , particularly in mental health, which is a sensitive and high-stakes domain.
Building on this notion of integration, it's crucial for designers and engineers to collaborate with domain experts. This collaboration allows for a deeper understanding of LLMs' capabilities and aligning expectations. Furthermore, such synergy can help mitigate over-reliance on technology and address the clinically relevant challenges~\cite{10.1145/3564752}. 

In this work, we present MindfulDiary, a mobile conversational AI for journaling that enables patients to record their daily experiences and thoughts through conversation. MindfulDiary incorporates LLMs to generate a response, prompting them differently according to the conversational phase. The conversation records are automatically summarized and presented on a clinician's dashboard so psychiatrists or clinicians can obtain insights about the patient. A multi-disciplinary research team, which included HCI researchers, engineers, and mental health professionals (i.e., psychiatrists and clinicians), carried out this project. We iteratively designed MindfulDiary, drawing insights from focus group interviews, expert evaluations of the chatbot's behaviors, and pilot studies.

To examine how patients interact with MindfulDiary, we conducted a four-week field study with 28 psychiatric patients and five psychiatrists at a university hospital. Patients performed journaling with MindfulDiary for four weeks, and their primary psychiatrists used the clinician's dashboard when they met their patients. The study revealed that the versatility, narrative-building capability, and diverse perspectives provided by MindfulDiary assist patients in consistently enriching their daily records. Furthermore, MindfulDiary supported patients in overcoming the challenges of detailed record-keeping and expression, often hindered by feelings of apathy and cognitive burdens. Notably, the enriched records from MindfulDiary, previously unattainable, provided psychiatrists with deeper insights, enhancing their understanding and empathy towards patients. Based on the findings, we discuss both the potential of LLMs' conversational abilities to aid in patient record-keeping within clinical mental health settings and suggestions for their responsible integration into these environments.

\npstart{The contributions from our research are as follows:}
\begin{enumerate}[leftmargin=*, itemsep=4pt, topsep=0pt]
    \item We present MindfulDiary, an LLM-driven journal designed to document psychiatric patients' daily experiences through naturalistic conversation developed in collaboration with mental health professionals.
    \item From a 28-day field study involving 28 patients and five psychiatrists, we provide empirical findings on how MindfulDiary supports patients in maintaining daily logs and assists psychiatrists in monitoring and comprehending patient states.
    \item Drawing from the design process of MindfulDiary and the findings of our deployment study, we outline key considerations and share lessons learned for the design and implementation of LLM's conversational capability in clinical mental health settings.
\end{enumerate}

%참고: This work forms part of a three-year, multi-disciplinary research collaboration thatcomprises a diverse team of researchers and developers with backgrounds in ML, Clinical Psychology,HCI, Design, Engineering and Data Compliance. Jointly, we investigate identified AI challenges in thecontext of SilverCloud Health0F1, an established iCBT platform for the treatment of depression, anxiety, andfunctional impairments [86].

%The authors of this paper include an HCI researcher, an AI engineer, and a university hospital professor. Additionally, ten medical professionals, comprising counselors and psychiatrists, collaborated on the development and deployment of MindfulDiary over eight months. The university hospital where this research took place is recognized as a tertiary hospital in Korea. In our work, we aimed to uncover the potential advantages and challenges of using LLMs in a clinical setting for mental health care, illustrated through the development and implementation of MindfulDiary. The subsequent section presents the formative study that served as the basis for the initial concept and design of our language model-based program.

% As underscored in Human-AI interaction design guidelines, the emphasis shouldn't solely be on "what new capabilities technologies like LLMs can offer" but rather on their intended purpose and the best way to utilize them in the given context~\cite{googlepair}. 

% Through the design of MindfulDiary, we explored how LLM capabilities, such as natural language understanding, summarization, and generation, can play a role in the mental health clinical setting. We conducted a field deployment study over four weeks with 28 patients and five psychiatrists. Through this, we were able to understand how the LLM-integrated MindfulDiary can be utilized in recording patients' daily logging and assisting mental health professionals in understanding and diagnosing patients.





\section{Related Work}
%수정중!
%상담에서 어떻게 질문을 하는지..

\subsection{Journal as a Patient-generated Health Data in Clinical Setting}
In our study, we emphasize the importance of Patient-Generated Health Data (PGHD) in clinical mental health settings. Specifically, we employ journals as a method for patients to chronicle their daily experiences, thereby utilizing these self-documented insights to enhance the mental health professional's patient understanding. 

PGHD has increasingly become an essential tool in clinical settings as it captures authentic, real-time insights into patients' health. According to RTI International, PGHD refers to \textit{"health-related data, such as health history, symptoms, biometric readings, treatment history, lifestyle choices, and other pertinent details, created, recorded, or gathered by patients or their designees"}~\cite{shapiro2012patient}. PGHD enhances communication between patients and clinicians and offers context around the patient, thereby heightening clinicians' awareness of patient health outside of regular clinical visits~\cite{10.1177/1460458220928184, cohen2016integrating}.

Within the mental health domain, PGHD can range from structured mental health assessments (\eg, anxiety, depression) to more unstructured data like mood-related symptoms and even social interactions tracking (\eg, social media use, number of calls)\cite{austin2020use, demiris2019patient, nghiem2023understanding}. Our study places particular emphasis on journals as a PGHD method in mental health settings. Journaling, as defined in PGHD studies, involves \textit{"the practice of writing down one's symptoms and other information related to one's daily life to discuss them during clinical appointments"}~\cite{figueiredo2020patient, zhu2016sharing}. By enabling patients to chronicle their daily experiences, journals present rich, self-documented insights that enhance the mental health professional's understanding of their patients.

However, while the benefits of journaling are clear, the act itself is not always straightforward. Writing about emotions and past experiences can be intricate, as individuals vary in their capacity to recognize, interpret, and articulate their feelings~\cite{salovey1990}. For some, especially those in psychotherapy, crafting a narrative that clarifies their life's journey and present concerns can be a challenging process~\cite{donnelly1991cognitive}. Additionally, many struggle with starting their entries, sticking to consistent journaling routines, and structuring their reflections~\cite{Travers2011}. 

Recognizing these challenges and opportunities that journaling has in mental health, our work with MindfulDiary aims to lower patients' burdens of documenting daily experiences and emotions. Furthermore, we investigate how journals can be utilized in clinical mental health care settings as a PGHD. Our study explores the promise of LLMs in natural language understanding and generation, specifically within the mental health domain. In the next section, we delve into integrating LLM technology in the mental health domain.











\subsection{LLMs for Mental Health Domain}
In the clinical field, artificial intelligence (AI) is driving new innovations. While it hasn't yet replaced healthcare professionals, it offers significant assistance in clinical decision-making, such as diagnosis and treatment~\cite{ref}. However, its adoption in the mental health field has lagged behind other health domains~\cite{10.1007/s11920-019-1094-0}. One of the reasons is that mental health relies more heavily on 'softer' techniques and subjective data, such as building relationships with patients and observing emotions and behaviors~\cite{10.1007/s40596-016-0627-7}. However, with the advancement of Natural Language Processing (NLP) – a subfield of AI focused on human-computer language interaction~\cite{jurafsky2000speech} – the mental health field is seeing more use of technology. This is particularly relevant as NLP's ability to interpret and grasp the subtleties of human speech aligns well with the importance of dialogue, sentiment, and expression in the mental health domain~\cite{calvo2017natural, demner2009can}. Building upon this capability, early applications of NLP have streamlined the summarization of therapy session notes, thereby enhancing clinicians' efficiency~\cite{perlich2015automatic}. Later, NLP began not only to extract emotional insights from therapist-client interactions~\cite{10.3758/s13428-020-01531-z} but also to predict symptoms of depression and anxiety~\cite{brockmeyer2015me}.

Recently, LLMs have gained attention in the mental health field. Trained on vast text data, they show exceptional performance and versatility, understanding intricate language patterns better than previous NLP models~\cite{ref}. Within the realm of mental health, LLMs, such as BERT, have surpassed traditional dictionary-based methods like LIWC in predicting sentiments during therapist-client therapy sessions~\cite{10.3758/s13428-020-01531-z}. However, LLMs, employing a neural network known as a "transformer" to generate outputs, come with inherent limitations tied to their mechanism~\cite{vaswani2017attention}. One key issue is the opacity of the process: it's challenging to discern how the model interprets a given input prompt. As a result, designers struggle to predict both the LLM's understanding of the input and the subsequent message it might produce~\cite{liu2023pre}.

Given the potential pitfalls of LLMs, it's crucial to address their limitations, especially within the delicate mental health domain. As indicated by \cite{10.1145/3564752}, there exists a significant gap between the technical feasibility of AI tools and their meaningful, responsible integration into clinical settings. Building on this knowledge, our paper focuses on the development and evaluation of MindfulDiary, aiming to showcase the use of LLM's conversational capability in real-world scenarios. By designing an LLM-based program specifically tailored for the mental health clinical setting and grounding its development in real-world requirements, we aspire to bridge the gap between the potential of LLMs and the practical needs of clinicians and patients.


\subsection{Designing Conversational Agents for Mental Health}
With the technological advancements in mental health care, applications of NLP for patient care are increasingly emerging. Among these applications, conversational agents, also known as chatbots, have gained prominence in the health domain. In mental health, chatbots not only provide mental health-related information but also facilitate therapeutic content such as cognitive behavioral therapy~\cite{woebot, 10.2196/12106, fulmer2018using}, expressive writing~\cite{park_chatbot}, behavioral reinforcement~\cite{10.2196/12106}, and solution-focused brief therapy~\cite{fulmer2018using}. Notably, the inherent nature of these digital agents, which operate without direct human involvement, can sometimes be more effective in mental health interventions than human counselors. For instance, individuals uncomfortable speaking candidly due to societal stigma may find communicating with chatbots more effective than with actual people~\cite{park_chatbot}. Furthermore, these digital solutions transcend temporal and spatial barriers, offering anytime, anywhere mental health support~\cite{cameron2019assessing}.

The design approach of these chatbots is largely divided into retrieval-based and generative-based~\cite{10.1109/icac347590.2019.9036844}. Many chatbots currently used for mental health therapy utilize a Retrieval-based approach~\cite{ABDALRAZAQ2019103978}. The basic principle of retrieval-based chatbots is to search for an appropriate response from a database based on natural language input from users. Since the responses and expected flow that the system can provide are already hard-coded in the database, chatbots can operate more consistently compared to generative-based ones. Such an approach, which is close to rule-based, is considered more responsible and secure~\cite{}. However, this method has several drawbacks. For instance, if a user enters a question that does not exist in the database, the chatbot may fail to respond. Thus, there is a limitation that designers or developers cannot flexibly respond in unforeseen situations. On the other hand, with the advancement of LLM technologies like GPT-3, a generative-based approach has made it possible to have chatbot systems that can produce coherent and contextualized outputs for any input, enabling open-domain dialogues~\cite{bae2022building}. 
% By leveraging "in-context learning," the system can process the dialogue history with users as input and generate responses relevant to the most recent interaction. A practical application of this strength is demonstrated in~\cite{wei2023leveraging}, where GPT-3 was utilized to design a chatbot. This bot, rather than delivering predetermined output, could engage users by asking them health-related questions (e.g., sleep, Exercise) through natural conversation.

Despite these breakthroughs, LLM-based systems inherently possess limitations, as detailed in Section 2.1. Past studies have reported specific issues with LLM-based chatbots in the mental health domain. For instance, a chatbot leveraging GPT-2 for mental health therapy occasionally generated non-word sentences or produced more negative outputs than positive ones~\cite{chatbot_review21}. Additionally, Replika, an LLM-based application intended for mental wellbeing, has occasionally displayed harmful content, exhibited inconsistent conversational styles, and faced challenges in accurately recalling user interactions, undermining its role as a long-term companion~\cite{10.48550/arxiv.2307.15810}.

Considering the inherent limitations of language models and given the delicate nature of mental health issues, we must reflect carefully on how and to what extent the conversational capabilities of these models should be utilized. Notably, previous studies have highlighted the potential risks of using language models as stand-alone replacements for therapeutic services, such as counselors~\cite{npj21}. In our research, we propose use cases in which the conversational abilities of LLMs can be seamlessly integrated into clinical settings. Specifically, we investigated how the conversational capabilities of LLMs could aid in documenting patients' daily experiences, providing clinicians with a deeper understanding of their patients.





%위의 선행연구들은 LLM의 대화능력이 정신건강 관리에 있어서 기회와 한계를 보여준다. 특히 chatGPT와 같이 완전한 open-domain dialog기반의 프로그램은 다양한 사용자의 요구들에 유연하고 능동적으로 반응할 수 있는 기회를 보여주고 있다. 하지만 언어모델이 가지는 inherent한 한계를 고려해볼때, 그리고, 정신건강이라는 민감한 주제를 다루는 상황에서, 언어모델의 대화능력을 어떤 목적으로 어디까지에 활용할 것인지에 대한 고민이 필요하다. 우리의 연구에서는 LLM의 conversation caapbility를 의료진에 의도한 목적에 활용할 수 있는 사용케이스를 제안하였으며, 특히 LLM의 유연한 대화능력이 사용자의 일상 기록에 있어서 어떤 도움과 역할을 할 수 있을지 탐구해보았다.

%이러한 챗봇들의 디자인 접근은 크게 retrieval-based와 generative-based로 나뉘어진다~\cite{10.1109/icac347590.2019.9036844}. 현재 많은 정신건강을 위한 치료용 챗봇은 Retrival based approach를 사용하고 있는데~\cite{ABDALRAZAQ2019103978}, 이러한 retrival based의 챗봇은 기본 원리는 사용자로 부터 받은 자연어 입력내용을 바탕으로 데이터베이스에서 적절한 응답을 검색하는 것이다. 시스템이 제공할 수 있는 응답과 예상되는 흐름이 이미 데이터베이스에 하드 코딩되어 있기 때문에, generative based에 비해 더 일관성 있게 동작하는 챗봇을 만들 수 있다. 때문에 이러한 rule-based에 가까운 접근은 보다 responsible하고 secure하다고 considered된다~\cite{}. 그러나 이 방법에는 여러 단점이 있다. 예를 들어, 데이터베이스에 존재하지 않는 질문을 입력하는 경우, 챗봇은 작업을 수행하는데 실패하게 될 수 있다. 때문에 디자이너나 개발자가 예상하지 못한 상황에서 유연하게 대응하는게 불가능하다는 한계가 있다.

%반면 최근의 GPT-3와 같은 LLM기술의 진보로 인해 generative-based 접근은 어떠한 입력에서도 coherent하고 contextualized 출력이 가능한, open-domain dialog가 가능한 챗봇 시스템을 가능하게 해주었다. LLM의 동작 원리 중 하나인 in-context learning을 활용하면 시스템은 사용자와의 대화 기록을 입력받아 대화 맥락 및 가장 최근 입력에 대응하는 결과를 출력할 수 있는데, 이처럼 LLM의 기술적 특성과 능력을 바탕으로 챗봇을 구축하는것은 가장 대표적인 LLM의 응용사례중 하나이다 (e.g., chatGPT). 하지만, 정신건강 도메인에서 LLM기반의 챗봇이 가지는 한계들도 보고되고 있다. 예를들어, GPT-2를 활용한 정신건강 therapy 챗봇이 non-word sentence를 생성하거나, 긍정적인 출력보다 부정적인 출력을 생성하기도 하였다~\cite{chatbot_review21}. 또한, metntal wellbeing을 위한 Replika의 경우 conversation style이 insonsistent하거나, 사용자와의 상호작용을 제대로 기억하지 못하는 모습으로 인해, consistent long-term companion으로서의 역할을 하지 못하는것으로 보고되기도 하였다~\cite{10.48550/arxiv.2307.15810}.

%위의 선행연구들은 LLM의 대화능력이 정신건강 관리에 있어서 기회와 한계를 보여준다. 특히 chatGPT와 같이 완전한 open-domain dialog기반의 프로그램은 다양한 사용자의 요구들에 유연하고 능동적으로 반응할 수 있는 기회를 보여주고 있다. 하지만 언어모델이 가지는 inherent한 한계를 고려해볼때, 그리고, 정신건강이라는 민감한 주제를 다루는 상황에서, 언어모델의 대화능력을 어떤 목적으로 어디까지에 활용할 것인지에 대한 고민이 필요하다. 우리의 연구에서는 LLM의 conversation caapbility를 의료진에 의도한 목적에 활용할 수 있는 사용케이스를 제안하였으며, 특히 LLM의 유연한 대화능력이 사용자의 일상 기록에 있어서 어떤 도움과 역할을 할 수 있을지 탐구해보았다.




%언어모델이 정신건강에 있어서 어떻게 활용되었고, 어떤 변화를 가져왔는지
%세션 노트 요약과 분석
%정신질환 탐색과 진단
%챗봇과 같은 intervention
%LLM이 등장하면서 멘탈헬스케어 분야에서도~




% - **NLP** is the overarching field concerned with the interaction between computers and human language.
% - **LMs** are statistical models used within NLP to predict word sequences.
% - **LLMs** are a specific type of LM characterized by their vast size and capability, often achieving state-of-the-art results in many NLP tasks.

% 1. **Natural Language Processing (NLP)**:
%     - **Definition**: NLP is a field of artificial intelligence (AI) that focuses on the interaction between computers and humans through natural language. The goal is to enable computers to understand, interpret, and generate human language in a way that is both meaningful and useful.
%     - **Scope**: NLP encompasses a wide range of tasks such as text classification, sentiment analysis, machine translation, speech recognition, information retrieval, and many more. It combines computational linguistics with computer science and cognitive psychology to process and analyze large amounts of natural language data.
  
% 2. **Language Model (LM)**:
%     - **Definition**: A language model is a type of statistical model used in NLP and computational linguistics. Its primary function is to determine the probability of a sequence of words occurring in a given language.
%     - **Application**: For instance, if you type in "I am going to the..." on your phone, a language model might predict "store" or "gym" as the next word. LMs are critical components in many NLP tasks, including machine translation, speech recognition, and text generation.
  
% 3. **Large Language Model (LLM)**:
%     - **Definition**: Large language models are a subset of language models that are trained on vast amounts of text data using deep learning techniques, particularly using architectures like transformers (e.g., GPT, BERT). These models have many more parameters compared to traditional language models.
%     - **Features**: Due to their size and the massive amount of data they're trained on, LLMs can generate coherent and contextually relevant sentences, paragraphs, or even longer texts. They can understand context, perform various tasks without task-specific training (known as few-shot or zero-shot learning), and are at the forefront of current NLP research and applications.
%     - **Example**: OpenAI's GPT-3 and GPT-4 are examples of LLMs.

%However, with the rise of Natural Language Processing (NLP), a subfield of AI focusing on human-computer language interaction~\cite{jurafsky2000speech}, there's increasing tech integration in the mental health domain. NLP's potential to decode and understand the nuances of human speech is especially important in the mental health domain, where dialogue, sentiment, and expression play crucial roles~\cite{calvo2017natural, demner2009can}. 




% Especially, challenges arise when considering how to seamlessly integrate PGHD into clinicians' workflows, manage and secure this data, and address concerns regarding the reliability of patient-collected data~\cite{cohen2016integrating, nundy2014using}. The extent and methodology of using PGHD, as well as how it's integrated into doctors' workflows, and the demonstration of best practices encompassing these, have been emphasized as needing further research in prior studies~\cite{wu2020clinician}. In our research, while designing MindfulDiary, we collaborated with mental health professionals. This collaboration encompassed the entire development process, including adjusting expectations regarding the system's development and technology, evaluation and improvement, and setting the purpose of use.

% In the mental health domain, types of PGHD range from mental health assessments (e.g., anxiety, depression), mood-related symptoms, Journaling to social interactions tracking (e.g., social media use, number of calls)\cite{austin2020use, demiris2019patient, nghiem2023understanding}. 

% In the PGHD, journaling which is defined by \textit{"the practices of writing down one’s own symptoms and other related information related to one’s daily life in order to later discuss them during clinical appointments"} ~\cite{figueiredo2020patient, zhu2016sharing}

% Yet, 

 % can be used for mental health management~\cite{10.1145/3025453.3025869}. 



% Understanding Mental Health Clinicians’ Perceptions and Concerns Regarding Using Passive Patient-Generated Health Data for Clinical Decision-Making: Qualitative Semistructured Interview Study~\cite{nghiem2023understanding}

% Patient-Generated Health Data: Dimensions, Challenges, and Open Questions~\cite{figueiredo2020patient}

% Sharing Patient-Generated Data in Clinical Practices: An Interview Study~\cite{zhu2016sharing}

% Clinician Perspectives and Design Implications in Using Patient-Generated Health Data to Improve Mental Health Practices: Mixed Methods Study~ \cite{wu2020clinician}

% Integrating Patient-Generated Health Data Into Clinical Care Settings or Clinical Decision-Making: Lessons Learned From Project HealthDesign~\cite{cohen2016integrating}

% Using patient-generated health data from mobile technologies for diabetes self-management support: provider perspectives from an academic medical center~\cite{nundy2014using}

% Quantifying the Body and Caring for the Mind: Self-Tracking in Multiple Sclerosis~\cite{10.1145/3025453.3025869}

% Patient diaries and patient-generated health data (PGHD) have been recognized as important tools in the clinical environment. Their importance stems from the dual purpose they serve: capturing authentic patient experiences in real-time and providing invaluable insights for clinicians to tailor their therapeutic interventions more precisely. A patient diary, employed during clinical trials or during the treatment of diseases, serves as a reliable method for clinicians to assess various aspects of a patient's condition, including symptom severity~\cite{stone2004understanding} and quality of life. It also aids in treatment compliance~\cite{van1999patient}. 


%Given the potential pitfalls of LLMs, it's crucial to address their limitations, especially within the delicate domain of mental health. As indicated by \cite{10.1145/3564752}, there's a significant gap between the technical feasibility of AI tools and their meaningful, responsible integration into clinical settings. Furthermore, the challenges in designing AI-infused systems have been previously highlighted by \cite{10.1145/3313831.3376301} due to their complexity and unpredictability compared to other HCI technologies. Building on this knowledge, our paper's focus on the development and evaluation of MindfulDiary aims to exemplify harnessing the LLM in the real world. By designing an LLM-based program tailored specifically for the mental health clinical setting and by grounding its development in real-world requirements, we aspire to bridge the gap between the potential of LLMs and the practical needs of clinicians and patients.
%Given these potential pitfalls of LLMs, it becomes important to address their shortcomings and limitations, especially within the sensitive context of mental health. Our paper's focus on the development and evaluation of MindfulDiary highlights the harnessing the LLM in the real-world. By designing an LLM-based program explicitly tailored for the mental health clinical setting, and by grounding its development in real-world requirements, we aim to bridge the gap between the potential of LLMs and the practical needs of clinicians and patients.

%이러한 LLM이 제공하는 기회와 한계는 언어모델을 정신건강 맥락에 적용할 때에 있어 많은 고민과 대비가 필요하다는 점을 보여준다. 특히, 정서적, 정신적으로 취약한 사람들이 사용하게 될 수 있는 mental health 분야에서 이러한 기술의 접목은 더욱더 주의깊고 세심하게 고려되어야 한다. 

%특히 선행연구에서도 predictability가 낮은 LLM과 같은 AI를 활용한 시스템 설계에 있어서, 이 기술이 어떤 capability를 가지는지에 대해 도메인전문가, 엔지니어, 디자이너가 공통된 이해수준을 가지는 것, 이러한 기술을 이용해 feasible한 프로그램을 만드는 데에 있어서 

% Furthermore, \cite{10.1145/3313831.3376301} has previously highlighted the challenges in designing AI-infused systems, emphasizing their complexity and unpredictability compared to other technologies. 

==> contents/delete_pilot_test.tex <==
% %내용 날리기
% \section{Pilot Study}
% We utilized an iterative design process, examining several prototype versions, and conducted a pilot study with eight mental health professionals and six patients to discover core usability issues and grasp the unexpected behavior of the LLM. 
% % One reason our iterative design process was particularly important was the importance of understanding how the LLM responds to patient utterances and the need for mental health professionals to verify and improve upon the LLM's behavior. Especially for generative models, considering their inherent limitation in predicting and controlling the behavior and output of the LLM, it was crucial to explore how we could systematically and effectively simulate and evaluate the model's outputs and pattern. In the following sections, we detail the approach taken to evaluate the MindfulDiary system.

% \subsection{Expert evaluation on LLM’s behavior}
% In this section, we introduce how we evaluate MindfulDiary by collaborating with five psychiatrists and three clinical psychologists. We conducted this assessment not only to determine how LLM responds to various patient utterances, particularly sensitive topics such as suicide and self-harm, but also to develop a common understanding between research teams regarding LLM's capabilities. Mutual understanding is critical for determining the target user group and the anticipated utility of MindfulDiary in a clinical setting.

% We conducted a prompt design workshop before the experts interacted with the LLM. Given the significance of prompt appropriateness to LLM outcomes, experts provided feedback on draft prompts, focusing on their clinical relevance and the embedded terminology and strategies. Next, the experts engaged directly with our LLM pipeline, simulating potential patient utterances. In order to better observe the model's output pattern and identify the problematic cases, we developed a test module that generates five responses with the same input. The experts can label concerning outputs and leave comments. We also evaluated the broader conversational flow using synthetic patient persona dialogues. In this evaluation, we generated dialogues using \textit{GPT-4} based on synthetic patient personas — developed in consultation with psychiatrists. This approach, involving 40 conversation sets, offered professionals a holistic view of conversation dynamics.

% These evaluation stages, beyond their primary purpose, allowed our research team to develop a mutual understanding of the LLM's capabilities. We made gradual updates based on the results of the iterative evaluation. The process allowed us to gain insight into the appropriate tone and manner of the LLM's outputs, as well as the appropriate length and flow of the conversation.

% %We described three evaluation methods to comprehensively assess the LLM's design and behavior. 

% % \subsubsection{Prompt Design Workshop}
% % In this section, we outline our workshop process that emphasizes a collaborative approach, actively engaging professionals in the design of MindfulDiary. Recognizing that the behavior and outcomes of the LLM's depend largely on the appropriateness of the prompts provided, we involved professionals in the design process to gain the expertise and knowledge they have. During the Prompt Design Workshop, clinicians were asked to read and give feedback on the given prompts. Their expert knowledge was instrumental in determining the prompts' appropriateness in a clinical setting. Furthermore, the workshop provided a platform for these professionals to evaluate the terminology and strategies embedded in the prompts. While the clinicians' evaluations did not necessarily lead to critical changes in the system, the workshop played a pivotal role in fostering understanding and alignment among different stakeholders during the system design.

% % \subsubsection{Direct Interaction-Based Evaluation with Medical Professionals}
% % In this evaluation, we let medical professionals directly interact with our LLM pipeline. By mimicking potential user(patient) utterances based on their clinical experiences, professionals assess the model's behavior and identify problematic scenarios. Especially, for a better understanding of how the model behaves we designed a test rig that can generate five responses with the same input so that professionals better observe the model's pattern and identify the problematic cases. This module also lets experts label problematic sentences that the model shouldn't generate and provides a text input field for qualitative feedback. Throughout the expert evaluation process, a total of xx sessions were assessed, and xxx pairs of input-LLM interaction were evaluated. Based on the evaluations, we used this module as a primary assessment tool and determined the model's appropriateness and potential usage.

% % \subsubsection{Evaluation Using Synthetic Patient Persona Dialogues}
% % Direct interaction with the language model is beneficial for understanding the model's behavior directly through simulating the patient. However, it's challenging and inefficient to comprehend the entire flow and progression of conversations. To address this issue, we generated dialogues with our LLM model based on synthetic patient personas. Especially in this process, we consulted psychiatrists to create patient personas that reflected the characteristics of despondent and cynical patients. These 40 conversation sets with these synthetic personas helped medical professionals grasp the flow and progression of dialogues and served as a supplementary tool to evaluations through interaction.



% \subsection{User evaluation of MindfulDiary}
% After the experts' evaluation of the LLM model and system, we conducted a pilot study targeting a potential user group. The pilot study was conducted in two main perspectives. Firstly, to understand if users easily understand the MindfulDiary program and to ensure there's no difficulty in its usage. Secondly, we aimed to understand how MindfulDiary's LLM outputs are generated and how users perceive them in real-world scenarios. The pilot study involved five patients who were currently admitted to a university hospital but were about to be discharged soon. 

% User evaluation was performed on a test platform designed to monitor the interaction between the patient and the system in real-time. The psychiatrists could preview and validate the generated output from LLM before it was delivered to the patient, thereby ensuring safeguards against potential hazards. Additionally, during this user evaluation process, experts could label problematic outputs for improvement as in the expert evaluation process. This served as an added checkpoint, enabling them to verify further if any potentially problematic responses were generated in line with expert assessments.

% Users found the prospect of using MindfulDiary for conversations and diary writing not only possible but also promising. Participants highly rated the LLM's utterances and questions, noting a significant difference from other apps. For example, one participant (P1-2) remarked, \textit{"While other apps felt like conversing with a machine, this felt like a genuine conversation with a human."} While there were noticeable differences in how users interacted with the system—varying interaction lengths and patterns—the majority of participants could smoothly engage in the session. Regarding areas of improvement, A recurrent theme was the need for a feature that allows users to obscure or hide diary entries, especially those with negative or dark content. Participants reflected on their past experiences, shedding light on why such a feature would be beneficial. P1-1 shared, \textit{"I had a previous experience with diary writing. Due to the prevalence of somber content, it often dampened my mood, leading me to abandon the practice."}. Additionally, participants underscored the need for understanding and assessing their own mental health. These needs have been incorporated and implemented in the system (\eg `save options', `Today's mental health' feature)
% % For instance, P1-2 mentioned that \textit{"It would be nice to have a feature that gives a score or an evaluation based on my diary, providing feedback on my mental state}.
% % % Furthermore, feedback touched on minor aspects like button design, labeling, and other usability concerns. 
% % These needs have been incorporated and implemented in the system (\eg `save options', `Today's mental health' feature)


% %의료진이 특히 주목해서 테스트와 관찰을 한 지점은 환자가 언급할 수 있는 explicit, implicit한 위험 신호나 메시지에 어떻게 언어모델이 동작하고, 우리의 모듈이 이를 잘 구분해내고 동작하는지 이해하는 것이였다. 먼저 우리는 module suggestion이 대화에서 위험신호를 파악하고 sensitive topic으로 이끌어내고, 의료진이 원하는 프로토콜로 잘 이끌고 갔었는지에 대한 부분이였다. 너무 많은 prompt

% %This shared knowledge ensured that clinicians could effectively utilize the tool in practice. One notable discovery was the inconsistency in the generated sentence lengths. Some outputs were excessively long, potentially creating cognitive burdens for patients. This variability was particularly pronounced when instructions on output length within prompts became less clear as input length increased. To mitigate this, we added instructions that solicited concise responses on the participant's last input, resulting in more consistent sentence lengths.  

% %대표적인 발견점을 얘기해보자면, 먼저 우리는 생성되는 문장의 길이가 일정하지 않은 경우를 먼저 발견할 수 있었다. 특히 exessive하게 길게 출력되는 문장들이 있었는데, 이러한 문장이 환자들의 인지에 부하가 될 우려를 언급했다. 특히, prompt에서의 출력 길이에 대한 instruction은 입력 양이 길어지며 그 의미가 희석되는 모습을 보였다. 우리는 이를 위해, 참가자의 마지막 입력에 출력의 길이를 1문장정도로 간결하게 요청하는 instruction을 add하였고, 길이의 조정에 있어 안정적으로 개선된 모습을 확인하였다. 의료진은 특히 환자가 언급할 수 있는 explicit, implicit한 위험 신호나 메시지에 어떻게 언어모델이 동작하고, 우리의 모듈이 이를 잘 구분해내는지 이해하는 것이였다. 자살/자해에 대한 처리는 애초에 gpt-4 모델이 위험한 방향으로 끌고가지 않았음. 사전에 잘 처리가 되어있는 것 같아보임. 우리가 원했던건 해당 상황 발생시 우리가 원하는 프로토콜로 잘 이끌고 갔었는지에 대한 부분. 이 부분에 있어서 언어모델이 어디까지 역할할 수 있을지에 대한 확인을 하였고, 언어모델의 동작이 안정적이고 의도에 맞는다고 합의되어 실제 환자를 대상으로 하는 pilot을 진행함. 또한 먼저 전문가들은 전문가들은 두가지 관점에서의 피드백을 제공해주었는데, 언어모델이 질문을 이끌어나가는 구조적인 관점, 언어모델이 가지는 늬앙스나 태도에 대한 의견이였다. 
% %특히 rule-based가 아닌 generative-based approach의 특성 상, 우리는 전문가의 모든 의견을 반영하기 어려운 한계를 인식할 수 있었다. 간단한 레벨의 질문 절차는 언어모델이 효과적으로 동작하는 것을 확인했지만, 

% %%Afterward, interviews to gather users' feedback on the program, a usability assessment (modified SUS), and a survey measuring the level of technological acceptance (UTAUT2) were carried out.

==> contents/figure.tex <==
%https://www.nami.org/About-Mental-Illness/Treatments/Types-of-Mental-Health-Professionals
%우리 프로그램 참여한 전문가: Mental Health Professionals
%상담사: Clinicians
%의사(전공의): Psychiatrists
%Mental Health Support
%Mental Health
%Clinical Mental Health Setting
%%도메인 관련 내용 추가하기!
%Patient Journaling의 문제 => LLM이 주는 새로운 기회 => LLM의 의학분야 적용에의 난점 => 우리가 한 것

% A journal serves as a written record of an individual's past events, thoughts, and feelings. A journal is unique because, usually, the person who writes it is the only one who reads it. This characteristic allows journals to be a safe place where writers can candidly express their concerns, thoughts, and emotions without the fear of judgment from others~\cite{Travers2011, Ullrich2002}. 


figure1 Figure 1: Image of MindfulDiary's interface split into two sections. On the left, the patient interface displays a journal session screen which aids user reflection through prompt question generation and journal-style summarization. On the right, the expert interface showcases a desktop dashboard layout, providing professionals with insights into journal interactions, key events and emotions, as well as the trend of PHQ-9 scores.
figure 2: Composite screenshot displaying four representative screens of the MindfulDiary patient interface. Starting from the far left: (a)A home screen featuring the user's name, recent journal entries count, and a button to initiate a session. (b) A screen captured during a journal session, showcasing a prompt question provided by MindfulDiary, a space for user's response, and a summarized journal entry. (c) A post-journaling summary screen displaying the user's current mental health status, the summarized journal entry, and a space for personal reflection. (d) A review screen where users can revisit their past journal entries, with entries visualized as individual cards.
figure 3: Sequential visual representation of the MindfulDiary's journaling session flow, depicted from left to right across four cards: (1) 'Pre-Journaling Assessment': Illustration of users taking a modified PHQ-9 mental health survey prior to their session with MindfulDiary. (2) 'User-MindfulDiary Conversation': Image of users engaging in a conversation with MindfulDiary, narrating and documenting their day. (3) 'Summary Presentation': Graphic depicting a diary-style summary of the three-turn conversation, with an option for users to edit. It signifies users' choice to either continue or end the conversation. (4) 'Session Closure': Visualization of the session's end screen, where MindfulDiary showcases the day’s mental health assessment alongside the diary content, signifying the conclusion of the journaling experience."
Figure 4: Visual representation of the MindfulDiary's conversational prompt pipeline, segmented into three distinct modules from left to right: (1) 'User Interaction': Depicts users engaging with and responding to MindfulDiary's messages. (2) 'Dialogue Analyzer': Shows the intake of the recent turn count, current state, and the entirety of the user-MindfulDiary dialogue. This module processes the conversation dynamics and is built upon the GPT-4 LLM framework. (3) 'Response Generator': Illustrates how the results from the Dialogue Analyzer, alongside a specified state prompt, summarization of the overall dialogue context, and the most recent three turns of the conversation, are inputted to produce a fitting response. This generated response is subsequently presented to the user. This module also operates on the GPT-4 LLM technology.
figure 5: Timeline diagram illustrating the progression of the field study in the research. Moving from left to right in chronological order: (1) 'Participant Recruitment', (2) "introductory session' (3) '4-week MindfulDiary Daily Use' (4) 'Surveys & Interviews': Three distinct markers or symbols at the beginning, middle (after 2 weeks), and end (after 4 weeks) of the usage period, highlighting the moments when surveys and interviews were conducted. (5) 'Researcher Monitoring'
table 1: "Table 1 presents a categorization of LLM’s strategies to produce prompts aimed at fostering user reflection. The table is structured into three columns: 'Category', 'Description', and 'Example'. 'Emotional Exploration': This category focuses on probing further into the user’s emotional state, mood, and condition. Sample questions include: “How did you feel after meeting her?” and “Can you tell me how this situation makes you feel?”. 'Activity Exploration': This strategy explores the user’s experiences or undertakings, leaning towards more factual content. For instance, questions such as “What kind of exercise do you do?” and “Lunch with a friend sounds nice. What did you eat?” fall under this category. 'In-depth follow-up': This category dives deeper into the root causes or reasons behind the user's moods, emotions, or particular situations. Example prompts include: “Since when have you felt this overshadowed mood?” and “If you feel confused, what might be the reason?”. 'Future Plan Exploration': Here, the emphasis is on how the user reacted or plans to tackle the events or emotions they've described. Example questions include: “That situation must have been challenging. Have you considered any solutions?” and “What have you done to alleviate the loneliness, even just a bit?”
table 2: Table 2 offers a summary of the diverse categories of input messages provided by participants. The table is segmented into three columns: 'Category', 'Description', and 'Example'. 'Emotional States': This category captures the variety of emotions the participants chronicled in their daily interactions. These emotions span a wide array, from negative to depressive feelings. Sample inputs include: “I’m so exhausted, I feel like I’m reaching my limit soon,” and “I’m very worried, scared, and anxious.” 'Events and Activities': This section includes mentions of events, tasks, or activities participants engaged in or observed, such as academic exams or travel. An example message is: “When I attended school, I got some walking in, but after vacation, I don’t have much reason to go out, leading to a decreased activity level.” 'Thoughts and Beliefs': Here, participants' thoughts, values, beliefs, and strong convictions are presented. This category especially encompasses thought patterns linked to mental health like distorted thinking. A representative message is: “I feel like someone is talking behind my back somewhere; they don’t like my actions and seem to exclude me.” 'Perceived Health Status': This category sheds light on participants' physical conditions, health misconceptions, reactions to medications, and their perceptions and behaviors concerning medication intake. Example inputs include: “I’ll starve and exercise to lose weight!” and “I just took my medicine, but it seems to be getting tasteless.” 'Relationships & Interactions': This section brings forward content concerning participants' relationships with others. It covers challenges rooted in interpersonal dynamics and the support and affirmation they receive from acquaintances. An exemplar message is: “I hated seeing my brother being happy. Forcing a cheerful tone also irked me.

==> contents/related_work_initial.tex <==
\section{Related Work}
In this section, we cover related work in two parts: (1) journal as a patient-generated health data, and (2) conversational agent for mental health.

\subsection{Journal as a Patient-generated Health Data in Clinical Setting}
PGHD---defined as \textit{``health-related data, such as health history, symptoms, biometric readings, treatment history, lifestyle choices, and other pertinent details, created, recorded, or gathered by patients''}~\cite{shapiro2012patient}---has increasingly become an essential tool in clinical settings to capture authentic, real-time insights into patients` health. Studies have shown that PGHD can enhance communication between patients and MHPs and offer contextual information about patients, thereby heightening MHPs' awareness of patient health outside regular clinical visits~\cite{10.1177/1460458220928184, cohen2016integrating, nundy2014using}.

Within the mental health domain, PGHD range from structured mental health assessments (\eg, anxiety, depression) to more unstructured data, including mood-related symptoms and social interactions tracking (\eg, social media use, number of calls)\cite{austin2020use, demiris2019patient, nghiem2023understanding}. Our study places particular emphasis on journals as a PGHD method in clinical mental health settings. Journaling refers to \textit{``the practice of writing down one`s symptoms and other information related to one`s daily life to discuss them during clinical appointments''}~\cite{figueiredo2020patient, zhu2016sharing}. Using a journal as a PGHD can particularly be useful in mental health contexts as it can offer rich, self-documented insights, which could improve MHPs` understanding of their patients~\cite{wu2020clinician}.

However, while the benefits of journaling are clear, the act itself is not always straightforward. Many people struggle with starting their entries, sticking to consistent journaling routines, and structuring their reflections~\cite{Travers2011}. Further, writing about emotions and past experiences can be intricate, as individuals vary in their capacity to recognize, interpret, and articulate their feelings~\cite{salovey1990, lane1990levels, luminet2004multimodal}. For some, especially in psychotherapy, crafting a narrative that describes one's life journey can be a challenging process~\cite{donnelly1991cognitive, pennebaker1999forming}. 

While previous research has extensively established the significance of employing journals as PGHD within clinical contexts, it is essential to acknowledge the inherent complexities tied to the journaling process. This becomes especially critical when contemplating its application within the specific demographic undergoing psychotherapy. With this background, our research explores the potential of LLMs in assisting the journaling process within the clinical mental health setting.

\subsection{Conversational Agent for Mental Health}
The field of artificial intelligence (AI) has proposed some significant innovations in medical settings, such as aiding clinical decision-making and diagnosis~\cite{magrabi2019artificial, beam2016translating}. However, AIs have rarely been integrated into mental health contexts, partly because the field has relied on nuanced techniques and subjective data, such as patient relationships and emotion observation~\cite{10.1007/s11920-019-1094-0, 10.1007/s40596-016-0627-7}. Recently, there has been a growing technological presence of Natural Language Processing (NLP) applications for supporting mental health, as NLP's capability for understanding human language holds a significant promise in this domain~\cite{calvo2017natural, demner2009can}.

Conversational agents, also known as chatbots, have particularly stood out in the mental health domain~\cite{abd2021perceptions, ABDALRAZAQ2019103978}. Studies have demonstrated the potential of chatbots in facilitating different types of therapy, such as cognitive behavioral therapy~\cite{woebot, 10.2196/12106, fulmer2018using}, expressive writing~\cite{park_chatbot}, behavioral reinforcement~\cite{10.2196/12106}, and solution-focused therapy~\cite{fulmer2018using}. Prior work has also shown that chatbots could ease the burden of disclosing sensitive information. Studies indicated that individuals may feel more comfortable communicating with chatbots because of the social stigma involved in communicating with human beings~\cite{10.1145/3313831.3376175, park_chatbot, 10.1145/3392836}. Furthermore, these approaches can help overcome temporal and spatial constraints, offering mental health support that is accessible at any time and anywhere~\cite{cameron2019assessing}.

Recently, chatbots powered by LLMs have gained attention~\cite{chatbot_review21}. Trained on vast amounts of text data, they demonstrate exceptional performance and versatility in natural open-domain conversation, surpassing previous NLP models in understanding intricate language patterns~\cite{radford2019language, 10.3758/s13428-020-01531-z}. Yet, many chatbots used for mental health therapy still employ a retrieval-based approach~\cite{ABDALRAZAQ2019103978, abd2019overview}. The basic principle of retrieval-based chatbots is to search for an appropriate response from a database based on input from users. Since the responses and expected flow that the system can provide are already hard-coded in the database, chatbots exhibit consistent and predictable behavior~\cite{10.1109/icac347590.2019.9036844}. However, if a user gives input that does not exist in the database, the chatbot may fail to respond. Thus, these systems cannot flexibly respond to unforeseen situations. In contrast, a generative approach driven by LLM has made it possible to develop chatbots that can produce human-like and contextualized outputs for even unforeseen input, enabling open-domain dialogues~\cite{bae2022building}. 

However, LLMs, employing a neural network known as a ``transformer'' to generate outputs, come with inherent challenges tied to their architecture~\cite{vaswani2017attention}. One key issue is the explainability of the model output: it's challenging to discern how this `black box' model interprets a given input prompt. As a result, designers struggle to predict both the LLM's understanding of the input and the subsequent messages it might produce~\cite{liu2023pre}. For instance, a chatbot leveraging GPT-2 for mental health therapy occasionally generated non-word sentences or produced more negative outputs than positive ones~\cite{chatbot_review21}. Replika, an LLM-based application intended for mental well-being, has occasionally displayed harmful content and exhibited inconsistent conversational styles, undermining its role as a long-term companion~\cite{10.48550/arxiv.2307.15810}. 

Considering the inherent challenges of LLM and the sensitivity of the mental health domain, we must reflect carefully on how and to what extent the conversational capabilities of these models should be utilized. In this study, we emphasize the need to consider the opportunities and limitations of LLMs, as well as important aspects of the mental health domain, including safety, sensitivity, and experts' empirical knowledge. With this in mind, we designed MindfulDiary's state-based chatbot using both rule-based and generation-based approaches to safe compliance with experts' guidelines while facilitating free-form conversations.

%In the following section, we introduce the formative study conducted with mental health professionals to create a clinically relevant system.

% Thus, in previous research, we can confirm the significance and potential of journals as PGHD in the clinical mental health setting. However, we also identified the limitation that the journaling process can sometimes be a complex process. Against this background, our research explores the promise of LLM in natural language understanding and generation, specifically within the clinical mental health setting. In the next section, we delve into integrating LLM technology into the mental health domain.

% Furthermore, with MindfulDiary, developed with real-world clinical use cases in mind, we aim to address the gap between the technical feasibility of AI tools and their clinically relevant, responsible integration~\cite{10.1145/3564752, npj21}. 

%이러한 배경에서 우리는, LLM이 가지고 있는 기회와 한계 (i.e.g, low predictability, consistency), 거기에 더해 정신건강 도메인에서 중요하게 다뤄져야 하는 safety, sensitivity, stretageis from clinical experience들이 복합적으로 고려되어야 한다는 점을 강조한다. 이를 위해, rule-based의 approach와 generation-based approach를 모두 활용한 state based의 시스템인 MindfulDiary를 설계하였다.
%또한 우리는 gap between the technical feasibility of AI tools and their meaningful, responsible integration into clinical settings~\cite{10.1145/3564752}을 adress하기 위해 챗봇의 역할에 있어 정신건강 지원을 대체하는 것이 아닌 보조적 수단으로 역할할 수 있는 실제 사례를 개발하고 배포하였다~\cite{npj}.

% Notably, previous studies have highlighted the potential risks of using language models as stand-alone replacements for therapeutic services, such as counselors~\cite{npj21}. In our research, we propose use cases in which the conversational abilities of LLMs can be seamlessly integrated into clinical settings. Specifically, we investigated how the conversational capabilities of LLMs could aid in documenting patients` daily experiences, providing clinicians with a deeper understanding of their patients.


% Given the potential pitfalls of LLMs, it`s crucial to address their limitations, especially within the delicate mental health domain. 

%In the clinical field, artificial intelligence (AI) is driving new innovations. While it hasn`t yet replaced healthcare professionals, it offers significant assistance in clinical decision-making, such as diagnosis and treatment~\cite{magrabi2019artificial, beam2016translating}. However, its adoption in the mental health field has lagged behind other health domains~\cite{10.1007/s11920-019-1094-0}. One of the reasons is that mental health relies more heavily on `softer` techniques and subjective data, such as building relationships with patients and observing emotions and behaviors~\cite{10.1007/s40596-016-0627-7}. However, with the advancement of Natural Language Processing (NLP) – a subfield of AI focused on human-computer language interaction~\cite{jurafsky2000speech} – the mental health field is seeing more use of technology. This is particularly relevant as NLP`s ability to interpret and grasp the subtleties of human speech aligns well with the importance of dialogue, sentiment, and expression in the mental health domain~\cite{calvo2017natural, demner2009can}. 


% As indicated by \cite{10.1145/3564752}, there exists a significant gap between the technical feasibility of AI tools and their meaningful, responsible integration into clinical settings. Building on this knowledge, our paper focuses on the development and evaluation of MindfulDiary, aiming to showcase the use of LLM`s conversational capability in real-world scenarios. By designing an LLM-based program tailored for the mental health clinical setting and grounding its development in real-world requirements, we aspire to bridge the gap between the potential of LLMs and the practical needs of clinicians and patients.


% \subsection{Designing Conversational Agents for Mental Health}
% With the technological advancements in mental health care, applications of NLP for patient care are increasingly emerging. Among these applications, conversational agents, also known as chatbots, have gained prominence in the health domain. In mental health, chatbots not only provide mental health-related information but also facilitate therapeutic content such as cognitive behavioral therapy~\cite{woebot, 10.2196/12106, fulmer2018using}, expressive writing~\cite{park_chatbot}, behavioral reinforcement~\cite{10.2196/12106}, and solution-focused brief therapy~\cite{fulmer2018using}. 

% The design approach of these chatbots is largely divided into retrieval-based and generative-based~\cite{10.1109/icac347590.2019.9036844}. 
% % By leveraging "in-context learning," the system can process the dialogue history with users as input and generate responses relevant to the most recent interaction. A practical application of this strength is demonstrated in~\cite{wei2023leveraging}, where GPT-3 was utilized to design a chatbot. This bot, rather than delivering predetermined output, could engage users by asking them health-related questions (e.g., sleep, Exercise) through natural conversation.

% Despite these breakthroughs, LLM-based systems inherently possess limitations, as detailed in Section 2.1. Past studies have reported specific issues with LLM-based chatbots in the mental health domain. 

% Considering the inherent limitations of language models and given the delicate nature of mental health issues, we must reflect carefully on how and to what extent the conversational capabilities of these models should be utilized. Notably, previous studies have highlighted the potential risks of using language models as stand-alone replacements for therapeutic services, such as counselors~\cite{npj21}. In our research, we propose use cases in which the conversational abilities of LLMs can be seamlessly integrated into clinical settings. Specifically, we investigated how the conversational capabilities of LLMs could aid in documenting patients` daily experiences, providing clinicians with a deeper understanding of their patients.




% Building upon this capability, early applications of NLP have streamlined the summarization of therapy session notes, thereby enhancing clinicians` efficiency~\cite{perlich2015automatic}. Later, NLP began not only to extract emotional insights from therapist-client interactions~\cite{10.3758/s13428-020-01531-z} but also to predict symptoms of depression and anxiety~\cite{brockmeyer2015me}.


%위의 선행연구들은 LLM의 대화능력이 정신건강 관리에 있어서 기회와 한계를 보여준다. 특히 chatGPT와 같이 완전한 open-domain dialog기반의 프로그램은 다양한 사용자의 요구들에 유연하고 능동적으로 반응할 수 있는 기회를 보여주고 있다. 하지만 언어모델이 가지는 inherent한 한계를 고려해볼때, 그리고, 정신건강이라는 민감한 주제를 다루는 상황에서, 언어모델의 대화능력을 어떤 목적으로 어디까지에 활용할 것인지에 대한 고민이 필요하다. 우리의 연구에서는 LLM의 conversation caapbility를 의료진에 의도한 목적에 활용할 수 있는 사용케이스를 제안하였으며, 특히 LLM의 유연한 대화능력이 사용자의 일상 기록에 있어서 어떤 도움과 역할을 할 수 있을지 탐구해보았다.

%이러한 챗봇들의 디자인 접근은 크게 retrieval-based와 generative-based로 나뉘어진다~\cite{10.1109/icac347590.2019.9036844}. 현재 많은 정신건강을 위한 치료용 챗봇은 Retrival based approach를 사용하고 있는데~\cite{ABDALRAZAQ2019103978}, 이러한 retrival based의 챗봇은 기본 원리는 사용자로 부터 받은 자연어 입력내용을 바탕으로 데이터베이스에서 적절한 응답을 검색하는 것이다. 시스템이 제공할 수 있는 응답과 예상되는 흐름이 이미 데이터베이스에 하드 코딩되어 있기 때문에, generative based에 비해 더 일관성 있게 동작하는 챗봇을 만들 수 있다. 때문에 이러한 rule-based에 가까운 접근은 보다 responsible하고 secure하다고 considered된다~\cite{}. 그러나 이 방법에는 여러 단점이 있다. 예를 들어, 데이터베이스에 존재하지 않는 질문을 입력하는 경우, 챗봇은 작업을 수행하는데 실패하게 될 수 있다. 때문에 디자이너나 개발자가 예상하지 못한 상황에서 유연하게 대응하는게 불가능하다는 한계가 있다.

%반면 최근의 GPT-3와 같은 LLM기술의 진보로 인해 generative-based 접근은 어떠한 입력에서도 coherent하고 contextualized 출력이 가능한, open-domain dialog가 가능한 챗봇 시스템을 가능하게 해주었다. LLM의 동작 원리 중 하나인 in-context learning을 활용하면 시스템은 사용자와의 대화 기록을 입력받아 대화 맥락 및 가장 최근 입력에 대응하는 결과를 출력할 수 있는데, 이처럼 LLM의 기술적 특성과 능력을 바탕으로 챗봇을 구축하는것은 가장 대표적인 LLM의 응용사례중 하나이다 (e.g., chatGPT). 하지만, 정신건강 도메인에서 LLM기반의 챗봇이 가지는 한계들도 보고되고 있다. 예를들어, GPT-2를 활용한 정신건강 therapy 챗봇이 non-word sentence를 생성하거나, 긍정적인 출력보다 부정적인 출력을 생성하기도 하였다~\cite{chatbot_review21}. 또한, metntal wellbeing을 위한 Replika의 경우 conversation style이 insonsistent하거나, 사용자와의 상호작용을 제대로 기억하지 못하는 모습으로 인해, consistent long-term companion으로서의 역할을 하지 못하는것으로 보고되기도 하였다~\cite{10.48550/arxiv.2307.15810}.

%위의 선행연구들은 LLM의 대화능력이 정신건강 관리에 있어서 기회와 한계를 보여준다. 특히 chatGPT와 같이 완전한 open-domain dialog기반의 프로그램은 다양한 사용자의 요구들에 유연하고 능동적으로 반응할 수 있는 기회를 보여주고 있다. 하지만 언어모델이 가지는 inherent한 한계를 고려해볼때, 그리고, 정신건강이라는 민감한 주제를 다루는 상황에서, 언어모델의 대화능력을 어떤 목적으로 어디까지에 활용할 것인지에 대한 고민이 필요하다. 우리의 연구에서는 LLM의 conversation caapbility를 의료진에 의도한 목적에 활용할 수 있는 사용케이스를 제안하였으며, 특히 LLM의 유연한 대화능력이 사용자의 일상 기록에 있어서 어떤 도움과 역할을 할 수 있을지 탐구해보았다.




%언어모델이 정신건강에 있어서 어떻게 활용되었고, 어떤 변화를 가져왔는지
%세션 노트 요약과 분석
%정신질환 탐색과 진단
%챗봇과 같은 intervention
%LLM이 등장하면서 멘탈헬스케어 분야에서도~




% - **NLP** is the overarching field concerned with the interaction between computers and human language.
% - **LMs** are statistical models used within NLP to predict word sequences.
% - **LLMs** are a specific type of LM characterized by their vast size and capability, often achieving state-of-the-art results in many NLP tasks.

% 1. **Natural Language Processing (NLP)**:
%     - **Definition**: NLP is a field of artificial intelligence (AI) that focuses on the interaction between computers and humans through natural language. The goal is to enable computers to understand, interpret, and generate human language in a way that is both meaningful and useful.
%     - **Scope**: NLP encompasses a wide range of tasks such as text classification, sentiment analysis, machine translation, speech recognition, information retrieval, and many more. It combines computational linguistics with computer science and cognitive psychology to process and analyze large amounts of natural language data.
  
% 2. **Language Model (LM)**:
%     - **Definition**: A language model is a type of statistical model used in NLP and computational linguistics. Its primary function is to determine the probability of a sequence of words occurring in a given language.
%     - **Application**: For instance, if you type in "I am going to the..." on your phone, a language model might predict "store" or "gym" as the next word. LMs are critical components in many NLP tasks, including machine translation, speech recognition, and text generation.
  
% 3. **Large Language Model (LLM)**:
%     - **Definition**: Large language models are a subset of language models that are trained on vast amounts of text data using deep learning techniques, particularly using architectures like transformers (e.g., GPT, BERT). These models have many more parameters compared to traditional language models.
%     - **Features**: Due to their size and the massive amount of data they`re trained on, LLMs can generate coherent and contextually relevant sentences, paragraphs, or even longer texts. They can understand context, perform various tasks without task-specific training (known as few-shot or zero-shot learning), and are at the forefront of current NLP research and applications.
%     - **Example**: OpenAI`s GPT-3 and GPT-4 are examples of LLMs.

%However, with the rise of Natural Language Processing (NLP), a subfield of AI focusing on human-computer language interaction~\cite{jurafsky2000speech}, there`s increasing tech integration in the mental health domain. NLP`s potential to decode and understand the nuances of human speech is especially important in the mental health domain, where dialogue, sentiment, and expression play crucial roles~\cite{calvo2017natural, demner2009can}. 




% Especially, challenges arise when considering how to seamlessly integrate PGHD into clinicians` workflows, manage and secure this data, and address concerns regarding the reliability of patient-collected data~\cite{cohen2016integrating, nundy2014using}. The extent and methodology of using PGHD, as well as how it`s integrated into doctors` workflows, and the demonstration of best practices encompassing these, have been emphasized as needing further research in prior studies~\cite{wu2020clinician}. In our research, while designing MindfulDiary, we collaborated with mental health professionals. This collaboration encompassed the entire development process, including adjusting expectations regarding the system`s development and technology, evaluation and improvement, and setting the purpose of use.

% In the mental health domain, types of PGHD range from mental health assessments (e.g., anxiety, depression), mood-related symptoms, Journaling to social interactions tracking (e.g., social media use, number of calls)\cite{austin2020use, demiris2019patient, nghiem2023understanding}. 

% In the PGHD, journaling which is defined by \textit{"the practices of writing down one’s own symptoms and other related information related to one’s daily life in order to later discuss them during clinical appointments"} ~\cite{figueiredo2020patient, zhu2016sharing}

% Yet, 

 % can be used for mental health management~\cite{10.1145/3025453.3025869}. 



% Understanding Mental Health Clinicians’ Perceptions and Concerns Regarding Using Passive Patient-Generated Health Data for Clinical Decision-Making: Qualitative Semistructured Interview Study~\cite{nghiem2023understanding}

% Patient-Generated Health Data: Dimensions, Challenges, and Open Questions~\cite{figueiredo2020patient}

% Sharing Patient-Generated Data in Clinical Practices: An Interview Study~\cite{zhu2016sharing}

% Clinician Perspectives and Design Implications in Using Patient-Generated Health Data to Improve Mental Health Practices: Mixed Methods Study~ \cite{wu2020clinician}

% Integrating Patient-Generated Health Data Into Clinical Care Settings or Clinical Decision-Making: Lessons Learned From Project HealthDesign~\cite{cohen2016integrating}

% Using patient-generated health data from mobile technologies for diabetes self-management support: provider perspectives from an academic medical center~\cite{nundy2014using}

% Quantifying the Body and Caring for the Mind: Self-Tracking in Multiple Sclerosis~\cite{10.1145/3025453.3025869}

% Patient diaries and patient-generated health data (PGHD) have been recognized as important tools in the clinical environment. Their importance stems from the dual purpose they serve: capturing authentic patient experiences in real-time and providing invaluable insights for clinicians to tailor their therapeutic interventions more precisely. A patient diary, employed during clinical trials or during the treatment of diseases, serves as a reliable method for clinicians to assess various aspects of a patient`s condition, including symptom severity~\cite{stone2004understanding} and quality of life. It also aids in treatment compliance~\cite{van1999patient}. 


%Given the potential pitfalls of LLMs, it`s crucial to address their limitations, especially within the delicate domain of mental health. As indicated by \cite{10.1145/3564752}, there`s a significant gap between the technical feasibility of AI tools and their meaningful, responsible integration into clinical settings. Furthermore, the challenges in designing AI-infused systems have been previously highlighted by \cite{10.1145/3313831.3376301} due to their complexity and unpredictability compared to other HCI technologies. Building on this knowledge, our paper`s focus on the development and evaluation of MindfulDiary aims to exemplify harnessing the LLM in the real world. By designing an LLM-based program tailored specifically for the mental health clinical setting and by grounding its development in real-world requirements, we aspire to bridge the gap between the potential of LLMs and the practical needs of clinicians and patients.
%Given these potential pitfalls of LLMs, it becomes important to address their shortcomings and limitations, especially within the sensitive context of mental health. Our paper`s focus on the development and evaluation of MindfulDiary highlights the harnessing the LLM in the real-world. By designing an LLM-based program explicitly tailored for the mental health clinical setting, and by grounding its development in real-world requirements, we aim to bridge the gap between the potential of LLMs and the practical needs of clinicians and patients.

%이러한 LLM이 제공하는 기회와 한계는 언어모델을 정신건강 맥락에 적용할 때에 있어 많은 고민과 대비가 필요하다는 점을 보여준다. 특히, 정서적, 정신적으로 취약한 사람들이 사용하게 될 수 있는 mental health 분야에서 이러한 기술의 접목은 더욱더 주의깊고 세심하게 고려되어야 한다. 

%특히 선행연구에서도 predictability가 낮은 LLM과 같은 AI를 활용한 시스템 설계에 있어서, 이 기술이 어떤 capability를 가지는지에 대해 도메인전문가, 엔지니어, 디자이너가 공통된 이해수준을 가지는 것, 이러한 기술을 이용해 feasible한 프로그램을 만드는 데에 있어서 

% Furthermore, \cite{10.1145/3313831.3376301} has previously highlighted the challenges in designing AI-infused systems, emphasizing their complexity and unpredictability compared to other technologies. 
